Embedding the Teacher: Distilling vLLM Preferences for Scalable Image Retrieval

Text--image retrieval is necessary for applications such as product recommendation. Embedding-based approaches like CLIP enable efficient large-scale retrieval via vector similarity search, but they are primarily trained on literal caption-like text--image pairs and often fail to capture abstract or persona-driven attributes common in product recommendation applications (e.g., ``a gift for a mother who loves gardening''). In contrast, state-of-the-art vision--language models (vLLMs) can align text with images in a flexible manner, but their limited context window prevents them from directly handling retrieval over large catalogs. We propose a framework that distills the preference rankings of a powerful vLLM into an embedding-based system, transferring its nuanced alignment abilities while maintaining the inference-time scalability of an embedding-based approach. Experiments on persona-driven product recommendation tasks demonstrate that our method significantly outperforms existing embedding-based baselines, providing an efficient solution for personalized text--image retrieval.

==> backup.tex <==
% Vision--language models (vLLMs) have shown strong performance in a range of multi-modal tasks~\cite{Gemini, Qwen, Llama}; for example: given a particular text prompt and a small candidate set of images, they can reliably select the most appropriate image conditioned on the prompt. However, when image selection is required from a large corpus of images,  a limit on the size of the context window prevents vLLMs from being a viable approach. This limitation is particularly relevant in real-world recommendation scenarios, where the query is a rich natural-language description of a persona and the candidate images are drawn from extensive product catalogs~\cite{MileBench}. For example, a user might ask: \emph{``My mum loves gardening, which Tiffany \& Co. bracelet (from a catalog) would she enjoy the most?''}. In such cases, the model must align abstract attributes of the text (``loves gardening'') with implicit associations in the catalog images.

    % \begin{figure}[htb!]
    %     \centering
    %     \includegraphics[width=1\linewidth]{intro.pdf}
    %     \caption{Comparison of methods for persona-based product image retrieval. vLLMs capture preferences well but cannot retrieve from a large catalog (context limit); CLIP enables retrieval but is not well aligned to product recommendation. Our approach distills vLLM preferences into an embedding-based approach to achieve both.}
    %     \label{fig:teaser}
    % \end{figure}


    % A common solution for large-scale text–image matching is to use embedding-based retrieval systems such as CLIP~\cite{CLIP}, ALIGN~\cite{jia2021scalingvisualvisionlanguagerepresentation}, or SigLIP~\cite{zhai2023sigmoidlosslanguageimage}. These models project text and images into a shared space, enabling efficient retrieval via vector similarity search. While effective for literal caption--image alignment (e.g., matching ``a red car'' to an image of a red car), they are less suitable when the text describes non-literal or persona-driven attributes, such as recommending gifts for a ``reserved mother'' or ``a student who enjoys hiking''. 

    % This gap is not only evident in persona-driven recommendation, but has also been highlighted more broadly in the context of visual retrieval. Recent evaluations of state-of-the-art image retrieval for visual RAG~\cite{visual-rag} find that existing embedding-based approaches often do not retrieve the best images. This is because such models are primarily trained on large-scale captioning datasets, which emphasize surface-level descriptions of visual content rather than abstract preferences or user intent~\cite{yuan2021florencenewfoundationmodel,luo2021clip4clipempiricalstudyclip}. Moreover, constructing labeled datasets that explicitly connect persona-style descriptions to product choices is prohibitively expensive, limiting the applicability of standard fine-tuning approaches.
    
    % In this work, we propose a practical framework to address the challenge of highly relevant retreival. Our approach (Figure~\ref{fig:teaser}) is to efficiently \emph{distill} the image preference rankings of a powerful vLLM into a lightweight embedding-based model. By supervising the embedding model with pairwise ranking signals derived from the vLLM, we enable large-scale, efficient recommendation through simple similarity search while retaining the nuanced, persona-driven alignment capabilities of the teacher vLLM. This approach addresses both scalability, by enabling fast inference over large catalogs, and adaptability, as it requires no manually labeled dataset of persona-to-product matches.
